Decomposable Submodular Maximization in Federated Setting

Submodular functions, as well as the sub-class of decomposable submodular functions, and their optimization appear in a wide range of applications in machine learning, recommendation systems, and welfare maximization. However, optimization of decomposable submodular functions with millions of component functions is computationally prohibitive. Furthermore, the component functions may be private (they might represent user preference function, for example) and cannot be widely shared. To address these issues, we propose a {\em federated optimization} setting for decomposable submodular optimization. In this setting, clients have their own preference functions, and a weighted sum of these preferences needs to be maximized. We implement the popular {\em continuous greedy} algorithm in this setting where clients take parallel small local steps towards the local solution and then the local changes are aggregated at a central server. To address the large number of clients, the aggregation is performed only on a subsampled set. Further, the aggregation is performed only intermittently between stretches of parallel local steps, which reduces communication cost significantly. We show that our federated algorithm is guaranteed to provide a good approximate solution, even in the presence of above cost-cutting measures. Finally, we show how the federated setting can be incorporated in solving fundamental discrete submodular optimization problems such as Maximum Coverage and Facility Location.

==> Acknowledgement.tex <==
\section*{Acknowledgement}
I would like to thank Arya Mazumdar and Barna Saha for their many useful discussions and for reading several drafts of this paper. I would also like to thank Yuichi Yoshida for his valuable discussions and inspiring comments on the paper. Additionally, I am grateful to Nazanin Mehrasa, Wei-Ning Chen, Heng Zhu, and Quanquan C. Liu for insightful comments on this work. 
